Diffusion Models as Cartoonists: The Curious Case of High Density Regions

We investigate what kind of images lie in the high-density regions of diffusion models. We introduce a theoretical mode-tracking process capable of pinpointing the exact mode of the denoising distribution, and we propose a practical high-density sampler that consistently generates images of higher likelihood than usual samplers. Our empirical findings reveal the existence of significantly higher likelihood samples that typical samplers do not produce, often manifesting as cartoon-like drawings or blurry images depending on the noise level. Curiously, these patterns emerge in datasets devoid of such examples. We also present a novel approach to track sample likelihoods in diffusion SDEs, which remarkably incurs no additional computational cost. Code is available at https://github.com/Aalto-QuML/high-density-diffusion.

==> sde_logp_diagram.tex <==
% \begin{tikzpicture}[
%   every node/.style={draw, rounded corners, align=center, minimum height=1.2em, font=\scriptsize},
%   box/.style={fill=blue!5, draw=blue!70, rounded corners, inner sep=0.5em, minimum height=1.5em, text width=10cm, align=center},
%   known/.style={draw=blue!70, rounded corners, inner sep=1em, thick, fill=blue!2, solid},
%   contribution/.style={draw=orange!70, rounded corners, inner sep=1em, thick, fill=orange!2, solid},
%   label/.style={font=\bfseries, align=left},
%   node distance=2cm and 10cm
% ]

% % Column Labels
% \node[font=\bfseries, minimum height=1.2em, text width=10cm, align=center] at (5,4.5) {Logp dynamics};

% % Known Results Group
% \node[known, fit={(ode_logp) (ode_logp)}, label={[label distance=2mm, label]north west:Known Results}] {};

% % Our Contribution Group
% \node[contribution, fit={(ftsde_logp) (rtsde_logp)}, label={[label distance=2mm, label]north west:Our Contribution}] {};

% % Row Labels
% \node[font=\bfseries, anchor=east, minimum height=1.2em] at (0,3) {ODE};
% \node[font=\bfseries, anchor=east, minimum height=1.2em] at (0,1) {Fwd SDE};
% \node[font=\bfseries, anchor=east, minimum height=1.2em] at (0,-1) {Rev SDE};

% % Grid Content
% % ODE Row (Known Result)
% \node[box] (ode_logp) at (5,3) {Insert ODE logp dynamics equation here};

% % Forward-time SDE Row (Our Contribution)
% \node[box, fill=orange!5, draw=orange!70] (ftsde_logp) at (5,1) {Insert Forward-time SDE logp dynamics equation here};

% % Reverse-time SDE Row (Our Contribution)
% \node[box, fill=orange!5, draw=orange!70] (rtsde_logp) at (5,-1) {Insert Reverse-time SDE logp dynamics equation here};

% \end{tikzpicture}


\begin{tikzpicture}[
  every node/.style={draw, rounded corners, align=center, fill=yellow!20, minimum height=1.2em, font=\scriptsize},
  box/.style={fill=green!20, draw, rounded corners, inner sep=0.5em, minimum height=1.5em, align=flush left},
  node distance=1.5cm and 6cm
]

% Column Labels
% \node[font=\bfseries, minimum height=1.2em] at (3,4.5) {State dynamics};
% \node[font=\bfseries, minimum height=1.2em] at (9,4.5) {Logp dynamics};

% Row Labels
\node[font=\bfseries, anchor=east, minimum height=1.2em] at (0,2.75) {ODE};
\node[font=\bfseries, anchor=east, minimum height=1.2em] at (0,0.5) {Fwd SDE};
\node[font=\bfseries, anchor=east, minimum height=1.2em] at (0,-1.5) {Rev SDE};

% Grid Content
% ODE Row
\node[box] (ode_state) at (6,3) {$d\vx_t = \left( f(t)\vx_t - \frac{1}{2}g^2(t) \nabla_\vx \log p_t(\vx_t) \right)dt$};
\node[box] (ode_logp) at (6,2.25) {$d \log p_t(\vx_t) = \left( -f(t)D + \frac{1}{2}g^2(t) \Delta_\vx \log p_t(\vx_t) \right)dt$};

% Forward-time SDE Row
\node[box] (ftsde_state) at (6,1.2) {$d \vx_t = f(t)\vx_t dt + g(t) d\rW_t$};
\node[box] (ftsde_logp) at (6,0.3) {$
d \log p_t(\vx_t) = \left( -f(t)D + \frac{1}{2}g^2(t) \| \nabla_\vx \log p_t(\vx_t) \|^2 + g^2(t)\Delta_\vx \log p_t(\vx_t) \right)dt$ \\ \hspace{50pt} $+ g(t) \nabla_\vx\log p_t(\vx_t)^T d \rW_t$};

% Reverse-time SDE Row
\node[box] (rtsde_state) at (6,-1) {$d \vx_t = \left(f(t)\vx_t -g^2(t) \nabla_\vx \log p_t(\vx_t) \right)dt + g(t) d\overline{\rW}_t$};
\node[box] (rtsde_logp) at (6,-1.9) {$d \log p_t(\vx_t) = \left( -f(t)D - \frac{1}{2}g^2(t) \| \nabla_\vx \log p_t(\vx_t) \|^2 \right)dt$  \\ \hspace{50pt} $ + g(t) \nabla_\vx \log p_t(\vx_t)^T d \overline{\rW}_t$};

\end{tikzpicture}


